Deep Exploration for Recommendation Systems

Modern recommendation systems ought to benefit by probing for and learning from delayed feedback. Research has tended to focus on learning from a user's response to a single recommendation. Such work, which leverages methods of supervised and bandit learning, forgoes learning from the user's subsequent behavior. Where past work has aimed to learn from subsequent behavior, there has been a lack of effective methods for probing to elicit informative delayed feedback. Effective exploration through probing for delayed feedback becomes particularly challenging when rewards are sparse. To address this, we develop deep exploration methods for recommendation systems. In particular, we formulate recommendation as a sequential decision problem and demonstrate benefits of deep exploration over single-step exploration. Our experiments are carried out with high-fidelity industrial-grade simulators and establish large improvements over existing algorithms.

==> env.tex <==
In this section, we introduce the open-source RS \textbf{Env}ironment set for \textbf{S}parse and \textbf{D}elayed feedback, \textbf{SDEnv}. The goal of the environments is to provide a testbed for researchers to study the behavior of algorithms in a RS environment with sparse and delayed feedback. Simulated environments are important to academic research in this field because sequential decision problems require responses from the environment after an action is applied and existing RS datasets are unable to produce counterfactual responses given the actions taken by an agent. We believe that the environments we provide in this work suit as a comprehensive evaluation benchmark for future reinforcement learning algorithms for Deep Exploration in RSs.

In the next two subsections, we provide two environments, the Toy Environment and the Yahoo Environment within the scope of SDEnv, that implement the framework described in Section 3.2. The Toy Environment is used for quick verification of algorithm correctness and the Yahoo Environment is used for experimenting with algorithms in high-fidelity simulation environment. Both environments offer an OpenAI Gym like API for actions and observations and are provided open-source \href{https://github.com/BillMatrix/deep_exploration_recsys}{\color{blue} \textbf{here}}. Note that to the best of authors' knowledge, there are only two pieces of literature that built a reinforcement learning simulator for RSs \cite{rohde2018recogym, ie2019recsim}. However, these simulators either update user state independently from recommendations given to the user or do not introduce sparsity in user feedback. Therefore they do not provide an environment with delayed and sparse feedback and is not well suited for testing the capability of algorithms under delay and sparsity, which are commonly observed in real-world RSs.

In the following subsections, we denote $\phi_e$ for the feature representation of the environment (the user of the RS), $\phi_A$ for the feature representation of the action and $\phi_t$ for the feature representation of the interaction history between the agent and the environment.
% \vspace{-0.1in}
\subsection{Toy Environment}
We start with a toy environment with sparsity and delay in feedback. At each time step, the agent has two actions to recommend to a user. Only if the agent apply the correct action throughout the entire episode, the agent is able to receive positive feedback. 

Following the definition in Section \ref{prob}, the maximum horizon $T = 7$ and the interest target $b = 5$. The toy experiment represents a decentralized RS environment where the environment does not change $\phi_e$ across episodes. The environment has a repository of $T$ recommendation units, ordered as $a_1, a_2, \dots, a_T$, and at each time step, the agent is presented with a set of units $\mathbf{A_t} = (\text{no-op}, a_t)$. These units are carefully designed such that
\begin{equation}
\vspace{-0.025in}
    g(\phi_e, \phi_{A_t}) = \begin{cases} 1 &\mbox{if } A_t = a_t \text{ and }t > T - b \\
    0 & \mbox{if } A_t = \text{no-op} \\
    -1 & \mbox{otherwise}\end{cases}. 
\vspace{-0.025in}
\end{equation}
The reward of the environment $r_t$ is defined as $r_t = \text{satisfied}_t$, where recall that $y_t = \sum_t g(\phi_e, \phi_{a_t})$ and $\text{satisfied}_t = \mathds{1}(y_t > b)$.

Here, for any $\epsilon$-greedy algorithms, the expected time to find an optimal solution is $O(2^T)$, where using Deep Exploration with Randomized Value Function, the expected time to find an optimal solution is $O(T)$, where $T$ is the time horizon \cite{osband2019deep}. 

The feature extraction process is the following. Since in the toy environment, $\phi_e$ does not influence the prediction model and hence we set it to be empty. $\phi_t$ is designed to be a vector with cardinality $T$, each entry represents a time step as the following.
\begin{equation}
    \phi_{t}[i] = 
        \begin{cases} 
            -1 &\mbox{if } i > t \\ 
            1 & \mbox{if $A_i = a_i$ at time step $i$} \\
            0 & \mbox{otherwise} \end{cases}.
\end{equation}

This experiment's setup is very similar to Example 1 of Section 4.1. At each time step, the agent has two actions to recommend to a user. Only if the agent applies the correct action throughout the entire episode, the agent is able to receive positive feedback. The only difference between this experiment and Example 1 is that each episode stops when user's interest falls below $0$. This is natural because usually when users receive irrelevant recommendations from a platform, they could quickly churn.
% \vspace{-0.1in}
\subsection{Yahoo Environment}
To fully understand the effectiveness of the models in the real world, we use \href{https://webscope.sandbox.yahoo.com/catalog.php?datatype=r&did=54&guccounter=1&guce_referrer=aHR0cHM6Ly93ZWJzY29wZS5zYW5kYm94LnlhaG9vLmNvbS8&guce_referrer_sig=AQAAAGYRV0ngSEGqPy8ohhBvn4DbjRoOd7QjJC2sb8vAN8_tQmHypSganV3Ya5mXAaOyrJS6DbCUa5tLZVeV8ejwewjoa_IyqPBefI0yrfb07hPaxuJ6oZqFVvaiW8LnmSZ7vM1utIJ32Gx0-bNg9gj-J8kkN4nOQP0C6ROP9304NzrP}{\color{blue} \textbf{Yahoo!'s front page today user click log dataset}} to create a real recommendation system simulation environment. This dataset provides labels of whether a user has clicked on a piece of content on Yahoo!'s front page.

For the Yahoo Environment, we still keep the general simulation framework defined in the section \ref{prob}, but with a few modifications based on the dataset. We train a click-through rate (CTR) classification model based on the dataset to generate the engagement intent from each user and unit pair and use the model as $g(\phi_e, \phi_a)$. This model is not visible to the agent. Reward of the environment is defined as $r_t = \text{satisfied}_t$, where recall that $y_t = \sum_t g(\phi_e, \phi_{a_t})$ and $\text{satisfied}_t = \mathds{1}(y_t > b)$ follows the definition in Section \ref{prob}, which indicates whether user's current interest is above the target interest level. $g$ is also normalized such that its 80th percentile is equal to 0. This is normalized to allow for user interest to go below 0. The normalized distribution simulate users' churning behavior as if a user turns of the platform after receiving irrelevant recommendations. Both $\phi_e$ and $\phi_a$ for each user and each unit are vectors with cardinality of 6 which is prepared by Yahoo! as features. 

Note that in generic RS environments, user's click feedback are in general immediately visible as a binary feedback. However, in this environment, we treat the probability produced by the classification model as an intent score for the user which accumulates to the user's satisfaction level. We purposefully hide such feedback from the agent such that the agent only observes feedback when the user is satisfied to create sparsity and delay in the environment. Such phenomenon is commonly observed in RS when optimizing for rating of a software, maximizing cumulative consumption time on a platform and many more scenarios. In this environment, the CTR classification model serves as a proxy to user's satisfaction level change and we acknowledge that in real production systems, the underlying dynamics could be more sophisticated. However, sequential decision problems require responses from the environment after an action is applied and existing RS datasets are unable to produce counterfactual responses given the actions taken by an agent. Since many researchers do not have access to interacting with real users in production systems, we hope that the simulation environment here fosters a testbed and a community for experimentation to advance the state-of-the-art algorithm optimizing for RS with sparsity and delayed consequences.

In the Yahoo Environment, we offer two different modes: 
% \vspace{-0.1in}
\subsubsection{Decentralized RS.} This environment also shares the same nature as Example 1, but in a more realistic setting, where a single user has to reach a certain high level of interest to give positive feedback. In this environment, we randomly sample a single user from Yahoo's dataset before each run of the experiment and run all algorithms with the following feature extraction method. We refer to this single user experiment as the decentralized RS environment. Note that since we use the same user for all algorithms, we set $\phi_e$ to be empty. $\phi_t$ is a vector with cardinality $6T$
\begin{equation}
    \phi_t[6i:6i+5] = 
        \begin{cases} 
            -\mathbf{1} &\mbox{if } i > t \\
            \phi_{a_i} & \mbox{if $a_i$ is used at time step $i$} \\
            \mathbf{0} & \mbox{otherwise} \end{cases}.
\end{equation}
where $-\mathbf{1}$ is a vector of six $-1$'s and $\mathbf{0}$ is a vector of six $0$'s. 

% \vspace{-0.1in}
\subsubsection{Centralized RS.} In this environment, we first sample $N$ users and create an environment where in each episode, all $N$ users simultaneously experience the simulated Yahoo frontpage. This environment is in nature similar to Example 2 in Section 4.1 where $N$ users experience an environment where they only provide positive feedback after hitting a certain interest level. The agent is allowed to learn across users to generalize a model to better personalize for every user. The feature update mechanism follows the same process described in Decentralized RS above.
